EAGR: Evidence-Guided Adaptive Graph Retrieval

Retrieval-Augmented Generation (RAG) for multi-hop reasoning requires retrieval to adapt as intermediate evidence reveals new information needs. Existing approaches support such retrieval through explicit graph structures or iterative query reformulation, introducing graph-construction or query-time overhead. We present Evidence-Guided Adaptive Graph Retrieval (EAGR), a framework in which accumulated evidence dynamically determines which semantic directions to explore next, and which requires no dedicated graph database and no explicit graph materialization. EAGR operates over an implicit semantic graph induced by compact passage metadata pre-ingested into a standard VectorDB. Starting from dense-retrieval seed passages, an LLM iteratively assesses accumulated evidence, identifies promising semantic directions, expands the retrieval frontier through metadata-based neighborhood lookup, and terminates once sufficient evidence has been collected. By precomputing semantic metadata, EAGR enables evidence-conditioned graph exploration without materializing an explicit graph, maintaining a dedicated GraphDB, or iteratively rewriting the query. Across three widely used multi-hop QA benchmarks, EAGR achieves the highest LLM-based answer accuracy among evaluated methods, outperforming the vanilla RAG by 17\% and strongest graph-aware baseline by 4\% percentage points averaged across three popular benchmarks HotPotQA, 2WikiMultiHopQA, and MuSiQue.

==> sections/tikzfig.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[
    font=\scriptsize,
    node distance=3.5mm and 3.5mm,
    box/.style={
        draw=gray!55,
        rounded corners=2pt,
        fill=blue!4,
        align=center,
        minimum height=7mm,
        inner sep=3pt
    },
    process/.style={
        box,
        fill=cyan!6
    },
    evidence/.style={
        box,
        fill=orange!7
    },
    output/.style={
        box,
        fill=green!7
    },
    arrow/.style={
        -{Latex[length=1.5mm]},
        draw=gray!75,
        line width=0.45pt
    },
    looparrow/.style={
        arrow,
        rounded corners=3pt
    }
]

% Initial retrieval
\node[box, minimum width=8mm] (query) {Query};
\node[process, right=of query, minimum width=18mm] (dense)
    {Dense\\retrieval};
\node[box, right=of dense, minimum width=18mm] (seeds)
    {Seed\\passages};

\draw[arrow] (query) -- (dense);
\draw[arrow] (dense) -- (seeds);

% Adaptive traversal
\node[process, below=5mm of seeds, minimum width=27mm] (assess)
    {Node Assessment\\+ Edge Selection};

\node[evidence, left=of assess, minimum width=22mm] (state)
    {Accumulated\\evidence $\mathcal{M}_t$};

\node[process, below=of assess, minimum width=27mm] (rank)
    {Evidence-Guided\\Edge Reranking};

\node[process, left=of rank, minimum width=22mm] (expand)
    {Graph\\Expansion};

\node[output, below=5mm of state, minimum width=22mm] (result)
    {Retrieved\\context};

\draw[arrow] (seeds) -- (assess);
\draw[arrow] (state) -- (assess);
\draw[arrow] (assess) -- node[right, font=\tiny] {selected edges} (rank);
\draw[arrow] (state.south) |- (rank.west);
\draw[arrow] (rank) -- (expand);

% Iterative expansion
\draw[looparrow]
    (expand.north) -- ++(0,2.5mm)
    -| node[pos=0.35, above, font=\tiny] {new passages}
    (assess.west);

% Early termination
\draw[arrow]
    (assess.south west) --
    node[sloped, above, font=\tiny] {sufficient}
    (result.north east);

\end{tikzpicture}

\caption{Overview of EAGR. Dense retrieval provides the initial seed
passages. EAGR then assesses passages, accumulates evidence, reranks selected
edge labels, and expands the implicit graph until sufficient evidence has
been retrieved.}
\label{fig:eagr-overview}
\end{figure}
